Experiment-driven Characterization of Full-Duplex Wireless Systems

We present an experiment-based characterization of passive suppression and active self-interference cancellation mechanisms in full-duplex wireless communication systems. In particular, we consider passive suppression due to antenna separation at the same node, and active cancellation in analog and/or digital domain. First, we show that the average amount of cancellation increases for active cancellation techniques as the received self-interference power increases. Our characterization of the average cancellation as a function of the self-interference power allows us to show that for a constant signal-to-interference ratio at the receiver antenna (before any active cancellation is applied), the rate of a full-duplex link increases as the self-interference power increases. Second, we show that applying digital cancellation after analog cancellation can sometimes increase the self-interference, and thus digital cancellation is more effective when applied selectively based on measured suppression values. Third, we complete our study of the impact of self-interference cancellation mechanisms by characterizing the probability distribution of the self-interference channel before and after cancellation.

==> 1-Introduction.tex <==
\section{Introduction}
% The very first letter is a 2 line initial drop letter followed
% by the rest of the first word in caps.
% 
% form to use if the first word consists of a single letter:
% \IEEEPARstart{A}{demo} file is ....
% 
% form to use if you need the single drop letter followed by
% normal text (unknown if ever used by IEEE):
% \IEEEPARstart{A}{}demo file is ....
% 
% Some journals put the first two words in caps:
% \IEEEPARstart{T}{his demo} file is ....
% 
% Here we have the typical use of a "T" for an initial drop letter
% and "HIS" in caps to complete the first word.

%%%%%
% ME commented out
%\IEEEPARstart{T}{his} demo file is intended to serve as a ``starter file''
%for IEEE journal papers produced under \LaTeX\ using
%IEEEtran.cls version 1.7 and later.
% You must have at least 2 lines in the paragraph with the drop letter
% (should never be an issue)
%I wish you the best of success.

% ME commented out

\IEEEPARstart{C}{urrent} deployed wireless communication systems employ either a time-division or frequency-division approach to bidirectional communication. This requires dividing the temporal and/or spectral resources into orthogonal resources and results in half-duplex wireless communication systems. The key deterrent in implementing a full-duplex wireless communication system, which consists on same band simultaneous bidirectional communication, is the large self-interference from a node's own transmissions in comparison to the signal of interest from the distant transmitting antenna. The large self-interference spans most of the dynamic range of the analog-to-digital converter in the receiving chain, which in turn dramatically increases the quantization noise for the signal of interest. However, recent experimental results for indoor scenarios have shown that it is possible to implement  self-interference cancellation mechanisms that can sufficiently attenuate the self-interference such that the resulting full-duplex wireless system can achieve higher rates than a half-duplex system \cite{Katti_Mobicom10,MyFDAsilomar}. Hence, recent results have demonstrated that full-duplex systems are a feasible option for future indoor wireless communications.


In this paper, we perform a data-driven analysis of the full-duplex architecture proposed in~\cite{MyFDAsilomar}. Based on extensive experimental data, our main contribution consists in characterizing the impact of different self-interference cancellation mechanisms on the performance of full-duplex wireless communication systems. We consider three methods to reduce self-interference, which can be classified as either \emph{passive} or \emph{active}. The passive suppression is simply attenuation caused by path-loss made possible by \emph{antenna separation} between the transmitting antenna and the receiving antenna on the same node. To reduce the dynamic range of the self-interference, we use the active \emph{analog cancellation} proposed in~\cite{MyFDAsilomar} where an additional RF chain is used to cancel the self-interference at the receiving antenna, before the  analog-to-digital converter. In addition, we also study active \emph{digital cancellation}, where the self-interference is removed in baseband after analog to digital conversion. Our characterization of total and individual cancellation mechanisms, based on extensive experimentations, shows that a total average cancellation of 74~dB can be achieved.


Our results show that the average amount of self-interference cancelled by active cancellation increases as the power of the self-interference signal increases. This result is intuitive because the canceller relies on estimating the self-interference channel, and a higher self-interference power implies lower channel estimation error and hence better cancellation. Our characterization of active cancellation as a function of the self-interference power allows us to show that for a constant signal to interference ratio (SIR) at the receiver antenna (this is the SIR before active cancellation), the rate of a full-duplex link increases as the self-interference power increases. This appears counter-intuitive at first but follows from the fact that the average amount of self-interference cancellation increases with increasing self-interference power. Related work on implementation of self-interference cancellation mechanisms \cite{Katti_Mobicom10,MyFDAsilomar,Katti_Mobicom11,DivisionFreeDuplex,FDMicrosoft} has reported measured values of the amount of cancellation that can be achieved but a characterization of the effect of increasing self-interference power on the amount of active cancellation and rate has not been reported before. Authors in~\cite{FDMicrosoft} have argued that the rate performance of full-duplex is independent of the transmitter power, this conclusion is valid for the particular model and implementation in~\cite{FDMicrosoft}, however we demonstrate that this doesn't generalize to all full-duplex implementations. Specifically, we demonstrate an implementation where the full-duplex rate increases as the transmit power increases. 

Related work \cite{Katti_Mobicom10,MyFDAsilomar,Katti_Mobicom11,DivisionFreeDuplex} has shown that digital cancellation, while by itself insufficient to deal with self-interference, can increase the total amount of cancellation when applied after analog cancellation. However, intuitively it is clear that in an ideal scenario where analog cancellation could achieve infinite dB of cancellation then having digital cancellation after analog cancellation would be unnecessary. This leads to the natural question regarding when is digital cancellation useful. We present results that show that the self-interference suppression achieved by digital cancellation when applied after analog cancellation decreases as the self-interference suppression achieved by analog cancellation increases. Further, our results show that when analog cancellation achieves large suppression then applying digital cancellation after analog cancellation can increase the noise in the system. No previous work on full-duplex system implementation has analyzed the performance of digital cancellation as a function of the performance of analog cancellation. Our results show that digital cancellation is an excellent ``safety net," i.e, for the cases when analog cancellation delivers poor suppression, digital cancellation is most useful when applied selectively frame-by-frame based on  measured suppression performance.

We complete our study of the full-duplex architecture in~\cite{MyFDAsilomar} by  characterizing the distribution of the self-interference channel before and after active cancellation. Before applying active cancellation the self-interference channel is the channel between two antennas that are close to each other, consequently there is a strong Line-Of-Sight (LOS) component and the magnitude of the self-interference channel can be modeled as a Ricean distribution with large $K$-factor. After applying active cancellation the strong LOS component is reduced, hence, the magnitude of the self-interference channel can be modeled as a Ricean distribution with smaller $K$-factor~\cite{HongVTC}. We present a characterization of the $K$-factor values before and after active cancellation, such characterization has not been reported before for any full-duplex architecture.

Full-duplex wireless communications have been considered in the context of two-way (bidirectional) communication~\cite{Katti_Mobicom10,MyFDAsilomar,Katti_Mobicom11,DivisionFreeDuplex,FDMicrosoft,HongVTC} and in the context of full-duplex relays~\cite{Riihonen2009,RiihonenDec2011,RiihonenSept2011}. Our analysis of the amount of self-interference cancellation achieved by the full-duplex architecture in~\cite{MyFDAsilomar} is applicable to full-duplex nodes either in a relay or a two-way communication scenario. Our analysis of the rate performance of full-duplex will focus only on a two-way system. 

The rest of the paper is organized as follows. In Section~\ref{sec:model_derivation} we derive equations that model the full-duplex architecture we have implemented and serve as a theoretical framework that we will use for explanation of our results. A description of the experiment setup is presented in Section~\ref{sec:experiment_setup}. In Section~\ref{sec:parameter_characterization} we present a characterization of the amount self-interference cancellation achieved and a characterization of the $K$-factor of the self-interference channel before and after active cancellation. In Section~\ref{sec:achievable_rates} we present an analysis of the achievable rate performance of full-duplex two-way systems. Conclusions are presented in Section~\ref{sec:conclusions}.



==> 6-Conclusions.tex <==
\section{Conclusions}
\label{sec:conclusions}

In order to advance the theory of full-duplex systems it is important to have signal models based on actual measurements. We contribute to this area by providing a characterization of the distribution of the self-interference before and after active cancellation mechanisms. We are the first ones to report a statistical characterization of the self-interference based on extensive measurements. 

We have characterized the effect of increasing self-interference and transmission power on the rate and cancellation performance of our full-duplex implementation. Such a characterization, while fundamental for the future deployment of full-duplex systems, is seldom provided in related work on full-duplex implementation. 

We are the first to characterize the performance of digital cancellation as a function of the performance of analog cancellation for a full-duplex implementation. The current belief in the literature has been that digital cancellation will always help improve the total cancellation. Further, it has some times been conjectured that the total analog plus digital cancellation would be equal to the sum of the cancellations measured independently in isolation. We demonstrate that when digital cancellation is preceded by analog cancellation, the amount of digital cancellation varies as a function of the amount of analog cancellation. Thus, only a full-system implementation can reveal the true benefits of combined analog and digital cancellation in an actual system. 

Finally, while our results are based on a single implementation of one full-duplex system, we believe our results analyze fundamental characteristics of full-duplex systems that had not been analyzed before.



